Practical Integer Overflow Prevention

Integer overflows in commodity software are a main source for software bugs, which can result in exploitable memory corruption vulnerabilities and may eventually contribute to powerful software based exploits, i.e., code reuse attacks (CRAs). In this paper, we present IntGuard , a tool that can repair integer overflows with high-quality source code repairs. Specifically, given the source code of a program, IntGuard first discovers the location of an integer overflow error by using static source code analysis and satisfiability modulo theories (SMT) solving. IntGuard then generates integer multi-precision code repairs based on modular manipulation of SMT constraints as well as an extensible set of customizable code repair patterns. We have implemented and evaluated IntGuard with 2052 C programs (approx. 1 Mil. LOC) available in the currently largest open- source test suite for C/C++ programs and with a benchmark containing large and complex programs. The evaluation results show that IntGuard can precisely (i.e., no false positives are accidentally repaired), with low computational and runtime overhead repair programs with very small binary and source code blow-up. In a controlled experiment, we show that IntGuard is more time-effective and achieves a higher repair success rate than manually generated code repairs.

==> disclaimer.tex <==
\textit{Contextual Disclaimer.}
This article is based on a paper published by Muntean et al.~\cite{muntean:integer},
which has been significantly extended with new results conducted in the field of
code reuse attacks prevention based on the initial publication as well as other recent work.
We added a new motivating example section which presents a C code snippet used 
to illustrate an integer overflow bug. This bug may lead to an Integer-Overflow to Buffer-Overflow
(IO2BO) error defined in the Common Weakness Enumeration (CWE-680)~\cite{cwe680}, to a buffer over-read or in some
cases to code reuse attacks. 
We showcase examples of a relatively new type of vulnerability and attack which can appear as the result of an integer overflow bug 
(i.e., Code Reuse Attacks (CRAs) with following types of attacks:
e.g.,
Jump Oriented Programming (JOP)~\cite{jop:bletsch}, 
Counterfeit Object-Oriented Programming (COOP)~\cite{schuster:coop},
Return Oriented Programming (ROP)~\cite{rop:buchanan}, etc.). 
Additionally, we added new related work (based on static, dynamic or hybride techniques which run on source or binary code)
which presents different approaches to detect integer
overflow bugs. Furthermore, we extended the discussion section were we
address current limitations of our tool and we give insight into future research steps.
Thus, the provided updates are useful in order to shed additional light on the obtained
results and on future research directions.

==> intro_old.tex <==
\todo[inline]{do this really at the end, see what parts can be reused w.r.t. issa15 paper} %ok
\todo[inline]{set the stage} %ok
\todo[inline]{What is the problem?}  %ok
\todo[inline]{Where are the other solutions lack?}  %ok
\todo[inline]{How do we address the problem?} %ok
\todo[inline]{What is our insight?} %ok
\todo[inline]{Why do we implemented our checker as an Eclipse plug-in?}  %ok
\todo[inline]{What are the benefits of using symbolic execution in this area?}  %ok
\todo[inline]{How do you envision your tool to be used? It should be used off-line and online by the developer in order to assist them in order to pinpoint errors. Mention this}  %ok
\todo[inline]{what is the purpose of measuring the runtime?}  %ok
\todo[inline]{The remainder of the paper is organized as follows.}  %ok
\todo[inline]{How does our approach improve the state-of the art of int. ov. patching approaches?}  %ok
\todo[inline]{What is our problem description, what is the problem?}  %ok
\todo[inline]{What is our technique, our new insight?}  %ok
\todo[inline]{What is the goal, why do we test on a benchmark and not on real programs?}  %ok
\todo[inline]{Be careful about false positive claims.} %ok
\todo[inline]{Use the motivating example in the technical description.} %ok
\todo[inline]{C modeling in prior works. What did other do? Why are we better than others?}  %ok
\todo[inline]{How is our tool better than other tools?} %ok
\todo[inline]{Is our tool classifying benign from exploitable integer overflows? no.} %ok
\todo[inline]{What about the detection of previously unknown int. overflow? How do we address this issue?}  %ok
\todo[inline]{What about systems that work on binary code, what are their advantages and disatvantages related to our work.} %ok
\todo[inline]{What are our contributions?} %ok
\todo[inline]{What about the detection of underflow/signedness and truncation, why do we focus only on the overflow. How can these other categories addressed by our too?} %ok
\todo[inline]{We annalyzed 2052 programs and our analysis is intra-procedural flow sensitive. State this from the beginning.} %ok
\todo[inline]{What about approximate path coverage? What do you mean with this in the section 4.2?} %ok
\todo[inline]{Avoid using not explained abreviations, CFG, CDT, etc.} %ok
\todo[inline]{Talk about the efforts of scalling to real programs. State why this is not our goal at first and what are the advantages and the dissatvantages of such tools. 
State what is our advantage and what others do.} %ok
\todo[inline]{State why the blow-up of the binary in some cases matter and why this is important in some scenarios.}  %ok
\todo[inline]{One of the main advantage of our tool and techniques is that it can help the user to detect int. overflows during development phase thus avoiding some scalability
issues which are usually encountered with real systems which have a higher complexity and thus make some static analysis methods easily reach to their limits.} %ok
\todo[inline]{For example the checker could be used in future as running all the time in background as the user types. The information can be cached and used afterwards
when the program gets bigger and bigger.} %ok
\todo[inline]{sections have to be added here.}  %ok
\todo[inline]{State how the patching of integer overflows influences the prevention of CRAs. Explain the needed requirements and how this influence such and cra.} %ok

% \textbf{0.The Big Picture.}
Integer overflows based vulnerabilities have threatened software programs for decades.
The deployment of various prevention mechanisms based on:
{static analysis for finding integer overflows}~\cite{targeted, sift, kint},
{runtime program repair}~\cite{diehard},
{benign integer overflows identification}~\cite{kint}, 
{directed and random fuzzing}~\cite{taintscope, buzzfuzz},
{concolic testing}~\cite{klee}, 
{library support and runtime checks}~\cite{safeint, integerlib}, and
{repair code transfer}~\cite{codephage} have helped to reduce the number of integer overflows.
But these tools have seen only little to no adoption in industry; partly because their benefits are
hard to be assessed in the context of real software projects~\cite{benefits}. 
Because of integer overflows and the potentially memory corruptions 
other security vulnerabilities~\cite{wang:intscope, kint} can manifest or can be 
exploited trough CRAs~\cite{rop:buchanan}.

% %motivational example
% \input{parts/example}

% \textbf{1.Problem.} 
Integer overflows are hard to be repaired and thus resulting memory corruptions are hard to be avoided for at least four main reasons.
First, integer overflows are of several types~\cite{brumley:rich}:
overflow~\cite{cwe190:overflow},
underflow~\cite{cwe191:underflow},
signedness~\cite{cwe195:signed},  
truncation~\cite{cwe197:truncation}, and illegal uses of shift operations.
% By shifting more positions than its bit width or a negative number of bits. 
% Note that this is similar to type casting which can lead to type confusion.
Second, integer overflows are typically exploited indirectly~\cite{brumley:rich}, through stack or heap overflows which can 
lead to buffer overflows. In contrast, buffer overflows can be exploited directly or indirectly.
Typical integer related vulnerabilities  (see Figure~\ref{Integer overflows reported over the last 10 years.}) lead to the following exploit types:
Denial of Service (DoS),
% \begin{figure}[ht!]
% \centering
%  \makebox[\columnwidth]{
%   \includegraphics[scale=1.08]{odt/distri.pdf}}
% %   \node[below=of img, node distance=0cm, yshift=1.2cm, xshift=.25cm, font=\color{black}] {Year};
% %   \node[left=of img, node distance=0cm, rotate=90, anchor=center,yshift=-.9cm,font=\color{black}] {\# Bad Type Casts Reported};
% \vspace{-.5cm}
% \caption{Integer- vs. buffer-overflow vulnerabilities.}
% \label{Integer overflows reported over the last 10 years.}
% \vspace{-.5cm}
% \end{figure}
\begin{figure}[ht!]
\centering
 \makebox[\columnwidth]{
  \includegraphics[scale=.7]{images/vulns.pdf}}
%   \node[below=of img, node distance=0cm, yshift=1.2cm, xshift=.25cm, font=\color{black}] {Year};
%   \node[left=of img, node distance=0cm, rotate=90, anchor=center,yshift=-.9cm,font=\color{black}] {\# Bad Type Casts Reported};
\vspace{-.5cm}
\caption{Integer related vulnerabilities reported by NVD.}
\label{Integer overflows reported over the last 10 years.}
\vspace{-.5cm}
\end{figure}
arbitrary code execution,
% \footnote{Figure~\ref{Integer overflows reported over the last 10 years.} depicts in logarithmic scale the number of integer overflows and the correlation to arbitrary code execution reports in the U.S. NVD~\cite{stats}.
% As of May 2017, U.S. NVD lists a total 949 integer overflows reports, 702 arbitrary code executions (ARB), 14 integer overflow based ACEs, 3772 buffer overflows, and 177 buffer overflow based ACE. These numbers show that while there is a relative comparable number of integer overflows and ACEs each year, the number of integer overflow based ACEs is relatively low. Also, note that the ratio between buffer- and integer-overflows is (3.97) while the ratio between buffer-overflow based ACEs and integer-overflow based ACEs is 12.6 over 10 years, respectively.
% This indicates that integer overflows are mostly exploited not directly~\cite{brumley:rich},
% but rather indirectly to generate subsequently a buffer overflow which can than lead to ACEs.
% These vulnerabilities were reported in apps such as Google's Chrome \& V8 JavaScript engine, Mozilla FF, Microsoft's IE 10, Edge \& Chakra JavaScript engine, \& iOS/OS X apps.},
bypass of an upper bound sanitization check, logic error, and array index attacks caused by a vulnerable integer value.
Third, integer overflows are hard to detect as these vulnerabilities can reside deep in the program, and manifest only for certain input types.
Finally, required integer overflow repair guarantees are hard to achieve. Reasons include that:
the location~\label{my:guarantees} where the generated integer overflow repair should be inserted is hard to determine;
generating the right repair format such that the repair is compilable, syntactically correct and does not change the program intended behavior is not trivial;
the overhead introduced by a repair is quite high if inserted na{\"i}vely in all integer overflow prone locations (particularly in hot code such as loops);
deciding if the integer overflow was correctly removed after inserting a repair is not well addressed;  
determining if the integer overflow manifest across multiple integer precisions is not trivial; and 
assessing if the integer overflow is intended or unintended is less researched.
% (\textit{i.e.,} all current solutions are based on a limited
% seeded input space which is used to determine if the integer overflow is intended or not).

% \textbf{2.Existing Solutions.}
Recent solutions which can be used to repair integer overflows statically are Sift~\cite{sift}, TAP~\cite{tap},
(commercial tools~\cite{commercial:tools} such as Coverity Static Analysis, CodeSonar, Klocwork Insight, Polyspace, and Infer) 
and dynamically SoupInt~\cite{soupint}, AIC/CIT~\cite{coker:integers}, CIntFix~\cite{CIntFix} rely on a variety of techniques depicted in Table~\ref{tab:truthTables:bla}.
Noticeable is that from this list only TAP first detects the integer overflow and than tries to remove it by repairing it. Thus the other tools may 
insert repairs that were not first categorized as real integer overflows, not propose repairs at all and as consequence may change the intended program behavior.
Further, the main challenges which are partially addressed by these tools which hindering their wide adoption are: their low precision w.r.t. false positives/negatives detection, 
their high runtime performance overhead (\textit{i.e.,} mostly the runtime based tools) and the generated repairs provide only few to no repair guarantees.
Thus, these repairs are highly unsafe and in the end useless.

Sift---to the best of our knowledge is the only sound repair tool---is a static input filter generation tool 
that inserts input filters in the program binary for which the source 
code was previously manually annotated with source code annotations.
This tool has the following limitations confirmed by the authors
(1) it relies on user source code annotations which are not always available to a source code program or require a considerable annotation overhead (\textit{e.g.,} annotating large code bases), 
(2) upper bound source code annotations for loops are needed when the analyzed expression depends on a not finite number of values,
(3) not all types of integer overflow relevant sites are supported (\textit{i.e.,} only memory allocations and block memory copy sites),
(4) for some type of applications (\textit{i.e.,} web servers, etc.) with no available input format specification (\textit{i.e.,} no image or video files) Sift can not be applied,
(5) the tool can not guarantee that unwanted program behavior is introduced since the filters may remove any integer overflow even intended ones, 
(6) does not support multi-precision integer overflow repairs, 
(7) annotated stub standard C library functions need to be provided upfront for functions which influence the computed symbolic condition (if not provided than the filter will not be generated), and
(8) can not help to avoid integer underflows even though it is straightforward to extend the algorithm to consider underflows as well.

% Further, for completeness reasons we acknowledge that CRAs can also be mitigated in many other ways not only memory corruption detection, \textit{i.e.,} layout disclosure prevention, code randomization, 
% control flow integrity (CFI), etc. However, we argue that the \textit{symbolic analysis based error prevention techniques have been unfairly forgotten} in favor of these other error-prone avenues geared towards 
% repairing zero-day vulnerabilities, but providing no soundness or completeness guarantees at all. %Detecting several zero-day bugs in a program is not sufficient for all security oriented projects.
% We further emphasize that CRAs should be addressed as early as possible \textit{and} in a frequent fashion during programming~\cite{early:repairs} 
% to tackle the root cause of CRAs (\textit{i.e.,} memory corruption). Testing frequently addresses the fact that most vulnerabilities are introduced 
% by a single commit and affect mostly only isolated parts of the modified code during programming~\cite{vcc}. In addition, this process should be 
% supported with usable tools made available to programmers for their daily routines. 

% \textbf{4.Our Idea and Novel Technique} 
In this paper, we introduce \textsc{IntGuard}, a tool for generation of useful and high quality integer overflow repairs.
\textsc{IntGuard} is non-intrusive and generates multi-precision sound integer overflow repairs based
on a conservative novel technique for automated generation of repairs for C source code which relies 
on satisfiability modulo theory (SMT) constraints solving. 
On one hand, \textsc{IntGuard}s goal is not to classify
integer overflows which can result in a memory corruption (\textit{e.g.,} if it is used to determine the size of a heap-buffer).
On the other hand, \textsc{IntGuard} can determine if an integer overflow is exploitable by performing an data flow analysis between a certain 
program source (\textit{i.e.,} user input) and a program sink (\textit{i.e.,} the source code location where the bug manifests).
Our novel technique relies on 
(1) static symbolic intra-procedural and context-sensitive source code analysis for error detection and repair, 
(2) a novel automated C source code repair generation algorithm based on SMT solving and code repair stubs, and 
(3) a semi-automatic repair insertion technique which satisfies our previously mentioned repair requirements without
the need to classify integer overflows (\textit{e.g.,} intended/unintended). 
We intend that the programmer uses \textsc{IntGuard} his daily routine~\cite{early:repairs} and that he is the final link in the repair insertion decision chain to account for very cautious 
vendors~\cite{vcc} which allow a code patch to be applied only after a thorough review.

More precisely, our integer overflow repair generation technique is based on modular manipulation of SMT constraints based on
deletion and insertion of new SMT constraints with the goal of generation new SMT constraint systems used for assessing if the generated 
repair satisfies some of the imposed repair requirements. Further, we build a 
static symbolic analysis engine for SMT constraints manipulation.

The \textit{soundness definition} we employ in this paper is as follows. 
The automatically generated code repairs are not program input dependent (\textit{i.e.,} SMT constraints and the Z3~\cite{z3:smt} solver are used).
The underling integer overflow detection checker generates no false negatives (\textit{i.e.,} every detected integer overflow is a genuine 
integer overflow, each program loop is unrolled up to 15 times, this value is customizable).
A program repair removes a previously detected integer overflow on all program execution paths, which reach the integer overflow location, without 
inserting unwanted program behavior (\textit{i.e.,} only the integer overflow is removed).

% \textbf{4.1 Repais characteristics.} 
Next to sound repairs, \textsc{IntGuard} fulfills the following two important objectives. 
First, \textsc{IntGuard} addresses four of the eight limitations of Sift: 
no source code annotations needed, 
can be applied to all types of C/C++ source code based programs, 
support for multi-precision repairs (\textit{i.e.,} five types of multi-precision repair types are supported), 
and the repairs can be used to avoid integer underflows.
Second, the generated repairs are syntactically correct (and thus compilable), and do not crash the program after insertion (\textit{i.e.,} do not introduce any unwanted program behavior). 
Finally, \textsc{IntGuard} checks for at least 54 types of integer overflows (see NSA's Juliet~\cite{juliet:test} test suite). 
Importantly, while repairs are generated fully automatically in an efficient fashion, the repair insertion can also be fully automated
if required.
To the best of our knowledge, there are currently no other techniques for repairing integer overflows in C source code, which satisfy all above stated guarantees, and as such our technique improves 
the state-of-the-art by statically inferring sound integer overflow repairs. 
% Furthermore, we provide the first static symbolic execution based technique for automatic generation of C source code repairs. 
% Similar to our work,~\cite{muntean:buffer} use a symbolic execution based technique to repair buffer overflows in C source code.


% \textbf{5.Decisions Made (clarifications).} 
% We decided to repair integer overflows since these---along buffer overflows---are mostly responsible for memory corruptions in C/C++ code. 
% Other types of integer overflow related problems (\textit{i.e.,} see~\cref{Integer Overflow Related Problems.} for more details) can be addressed similarly
% since only the program site differs and the bug triggering condition (i.e., overflow, underflow, truncation, etc.) which can be easily added to \textsc{IntGuard}
% to be taken into consideration.
% We analyze source code rather than binary code or an intermediate representation (IR) since source code is semantically more richer.
% We envision that our tool will be used both online 
% % (\textit{e.g.,} can mitigate some application scalability issues) 
% and likewise offline by developers depending on their needs and usage scenarios.
% \textsc{IntGuard} uses symbolic execution and SMT solving for generating code repairs due to the fact that these techniques offer high precision for the locations 
% where the repair has to be inserted. In addition to that, the repair inference is input independent and the repair logic can be easily checked if it meets the repair acceptance
% criteria (\textit{i.e.,} see our nine repair guarantees). 
% Moreover, we tested \textsc{IntGuard} on benchmark programs for three main reasons: 
% \textit{(i)} to better compare it to other state-of-the-art tools, 
% \textit{(ii)} to measure more accurately its precision and repair inference quality (\textit{i.e.,} all integer overflows are known upfront, see Juliet benchmark particularities~\cite{juliet:test}), and 
% \textit{(iii)} the benchmark programs cover most control flow situations where integer overflow occur.
% % Note that detection of previously unknown integer overflows is out of scope of our current research since these type of errors are hard to assess. 
% % That is because there is no upfront common known ground truth available. 
% \textsc{IntGuard} can efficiently scale to larger programs since our loop unrolling analysis is of fixed customizable depth (\textit{i.e.,} 10 times) and the list of used function 
% summaries can be updated beforehand.
% The trade-off of \textsc{IntGuard} towards scalability is that the tool looses precision when dealing with recursion or loops but nevertheless the 
% repairs remain sound since these are not input dependent.
% Finally, the effectiveness, precision and practicability of the automatically generated repairs are our primary goals.

% \textbf{6.Evaluation.} 
In our evaluation, we analyzed 2052 C programs representing $\approx$1 Mil. LOC and have shown that~\textsc{IntGuard} repairs 
more programs on the same test suite across multiple integer precisions than CIntFix~\cite{CIntFix}, while inducing only
around 1\% computational overhead and ($\le$2\%) runtime performance overhead, respectively.
CIntFix and AIC/CIT~\cite{coker:integers} induced 16\% and above 30\%, runtime overhead, respectively.
The program binary and source code blow-ups of the repaired programs are insignificant ($\le$1\%). 
Further, we construct a mini-benchmark which we used to asses the precision and efficiency of our tool w.r.t. large and complex programs.
In the evaluation we showed that \textsc{IntGuard} scales to large programs and that our tool is efficient w.r.t. bug detection and repair generation.
In contrast, to other similar tools which only look to achieve scalability w.r.t. large programs we also search to detect and repair large programs in a systematic way.
Thus, this qualifies \textsc{IntGuard} for real life application.
% such as usage in embedded scenarios where size of the binary is key or in performance-oriented programs. 
Finally, we present several \text{in-the-wild} integer overflow types which can potentially be avoided if \textsc{IntGuard} is used throughout 
programmer's daily routines.

% \textbf{7.Contributions.} 
In summary, we make the following contributions: 
% \vspace{-.3cm}
\begin{itemize}[leftmargin=.3cm]

% \textbf{Novel Code Repair Technique.}
%  \item  We design a novel source code repair generation technique which is superior to other state-of-the-art techniques
%         due to its precision and provided repair guarantees.

\item  We designed a novel sound integer overflow C source code repair generation technique.
  
  %  \textbf{Usable Prototype.} 
%  \item We implemented \textsc{IntGuard}, a tool based on a novel integer overflow repairing technique, for C/C++ source code programs which 
%  we will make open source.
%  are open source: \url{https://github.com/domain/IntGuard}.

 \item We implemented \textsc{IntGuard}, a tool based on our novel integer overflow repairing technique.

%   \textbf{Integer Multi-precision Repair Tool.} 
%  \item We provide the first usable open-source C source code repair tool that can be used to repair integer overflows across multiple integer precisions.

 \item We provided the first open-source repair tool that can be used to repair integer overflows across multiple integer precisions.

 %  \textbf{More Useful Repair Guarantees.} 
%  \item We demonstrated trough extensive experiments that \textsc{IntGuard} is substantially more precise, effective 
%        and provides more useful repair guarantees than other state-of-the-art integer overflow repair tools.
  \item We experimentally demonstrated that \textsc{IntGuard} is superior to other state-of-the-art integer overflow repair tools.
       
%  \textbf{Evaluation.} 
%  \item We evaluate \textsc{IntGuard} thoroughly against the currently largest open-source test suite for C/C++ source code (NSA's Juliet) testsuite 
%  and show that the generated code repairs are effective, precise and induce low runtime overhead. Further, we designed a mini-benchmark
%  for assessing how \textsc{IntGuard} scales w.r.t. bug search in complex programs. 
 \item We evaluated \textsc{IntGuard} thoroughly and show that it is effective and scales to large programs.
%  
%  \textbf{Controlled Experiment.} 
%  \item We conducted a controlled experiment in which we show that \textsc{IntGuard} is up to 18 times more time effective than 
%        manual repairs.
 
 \item We showed that \textsc{IntGuard} is considerably more time effective than manual repairs generation and insertion.
%        At the same time, 84\% of the participants found our tool highly usable and 73\% of the participants would further recommend it.
\end{itemize}





